Computing Stackelberg Equilibria of Large General-Sum Games

We study the computational complexity of finding Stackelberg Equilibria in general-sum games, where the set of pure strategies of the leader and the followers are exponentially large in a natrual representation of the problem. In \emph{zero-sum} games, the notion of a Stackelberg equilibrium coincides with the notion of a \emph{Nash Equilibrium}~\cite{korzhyk2011stackelberg}. Finding these equilibrium concepts in zero-sum games can be efficiently done when the players have polynomially many pure strategies or when (in additional to some structural properties) a best-response oracle is available~\cite{ahmadinejad2016duels, DHL+17, KV05}. Despite such advancements in the case of zero-sum games, little is known for general-sum games. In light of the above, we examine the computational complexity of computing a Stackelberg equilibrium in large general-sum games. We show that while there are natural large general-sum games where the Stackelberg Equilibria can be computed efficiently if the Nash equilibrium in its zero-sum form could be computed efficiently, in general, structural properties that allow for efficient computation of Nash equilibrium in zero-sum games are not sufficient for computing Stackelberg equilibria in general-sum games.

==> figs/reduction1.tex <==

\begin{figure}[h!]
%\begin{minipage}{0.9\textwidth}
%\centering
\hspace*{-1cm} \begin{tikzpicture}[node distance=1.3cm,>=stealth',bend angle=45,auto,scale=0.8]

\tikzstyle{place}=[circle,thick,draw=blue!75,fill=blue!20,minimum size=6mm]
\tikzstyle{red place}=[place,draw=red!75,fill=red!20]
\tikzstyle{transition}=[rectangle,thick,draw=black!75,
fill=black!20,minimum size=4mm]

\tikzstyle{every label}=[red]

\begin{scope}[shift={(-1,0)}]

\node [place] at (-3,-3.1)(w1)                                                {};
\node [place] at ($(w1)+(0.8,0)$) (w2)                                              {};
\node  at ($(w2)+(0.7,0)$)  {$\ldots$};
\node [place] at ($(w2)+(1.4,0)$) (w3)                                              {};
\node  at (w3)  {$a$};
\node  at ($(w3)+(0.7,0)$)  {$\ldots$};
\node [place] at ($(w3)+(1.4,0)$) (w4)                                              {};
\node [place] at ($(w4)+(0.8,0)$) (w5)                                              {};
\draw ($(w1) + (-0.4,0.6)$) -- ($(w5) + (0.4,0.6)$) -- ($(w5) + (0.4,-0.6)$) -- ($(w1) + (-0.4,-0.6)$) -- cycle;
\node  at ($(w3)+(0,-1)$)  {$A$};

\begin{scope}[shift={(-5,3.7)},rotate=45]
\node [place] at (-3,-3.1)(g1)                                                {};
\node [place] at ($(g1)+(0.8,0)$) (g2)                                              {};
\node [rotate = 45] at ($(g2)+(0.7,0)$)  {$\ldots$};
\node [place] at ($(g2)+(1.4,0)$) (g3)                                              {}
edge [thick]                 (w3);
\node [rotate = 45] at (g3)  {$b$};
\node [rotate = 45] at ($(g3)+(0.7,0)$)  {$\ldots$};
\node [place] at ($(g3)+(1.4,0)$) (g4)                                              {};
\node [place] at ($(g4)+(0.8,0)$) (g5)                                              {};
\draw ($(g1) + (-0.4,0.6)$) -- ($(g5) + (0.4,0.6)$) -- ($(g5) + (0.4,-0.6)$) -- ($(g1) + (-0.4,-0.6)$) -- cycle;
\node [rotate = 45]  at ($(g3)+(0,1)$)  {$B$};
\end{scope}

\begin{scope}[shift={(4.6,2.57)},rotate=-45]
\node [place] at (-3,-3.1)(h1)                                                {};
\node [place] at ($(h1)+(0.8,0)$) (h2)                                              {};
\node [rotate = -45] at ($(h2)+(0.7,0)$)  {$\ldots$};
\node [place] at ($(h2)+(1.4,0)$) (h3)                                              {}
edge [thick]                 (w3)
edge [thick]                 (g3);
\node [rotate = -45] at (h3)  {$c$};
\node [rotate = -45] at ($(h3)+(0.7,0)$)  {$\ldots$};
\node [place] at ($(h3)+(1.4,0)$) (h4)                                              {};
\node [place] at ($(h4)+(0.8,0)$) (h5)                                              {};
\draw ($(h1) + (-0.4,0.6)$) -- ($(h5) + (0.4,0.6)$) -- ($(h5) + (0.4,-0.6)$) -- ($(h1) + (-0.4,-0.6)$) -- cycle;
\node [rotate = -45]  at ($(h3)+(0,1)$)  {$C$};
\end{scope}



\end{scope}

\begin{scope}[xshift=6cm]

% Second net
\node [place] (w1')                                                {};
\node [place] at ($(w1')+(0.8,0)$) (w2')                                              {};
\node  at ($(w2')+(0.7,0)$)  {$\ldots$};
\node [place] at ($(w2')+(1.4,0)$) (w3')                                              {};
\node  at (w3')  {$a'$};
\node  at ($(w3')+(0.7,0)$)  {$\ldots$};
\node [place] at ($(w3')+(1.4,0)$) (w4')                                              {};
\node [place] at ($(w4')+(0.8,0)$) (w5')                                              {};
\draw ($(w1') + (-0.4,0.6)$) -- ($(w5') + (0.4,0.6)$) -- ($(w5') + (0.4,-0.6)$) -- ($(w1') + (-0.4,-0.6)$) -- cycle;
\node  at ($(w3')+(0,1)$)  {$A'$};

\node [place] (g1') at ($(w1')+(0,-3)$)                                           {};
\node [place] at ($(g1')+(0.8,0)$) (g2')                                              {};
\node  at ($(g2')+(0.7,0)$)  {$\ldots$};
\node [place] at ($(g2')+(1.4,0)$) (g3')                                              {}
edge [thick]                 (w3');
\node  at (g3')  {$b'$};
\node  at ($(g3')+(0.7,0)$)  {$\ldots$};
\node [place] at ($(g3')+(1.4,0)$) (g4')                                              {};
\node [place] at ($(g4')+(0.8,0)$) (g5')                                              {};
\draw ($(g1') + (-0.4,0.6)$) -- ($(g5') + (0.4,0.6)$) -- ($(g5') + (0.4,-0.6)$) -- ($(g1') + (-0.4,-0.6)$) -- cycle;
\node  at ($(g3')+(0,-1)$)  {$B'$};

% Second net
\node [place] (h1') at ($(w5')+(1,0)$)                                           {};
\node [place] at ($(h1')+(0.8,0)$) (h2')                                              {};
\node  at ($(h2')+(0.7,0)$)  {$\ldots$};
\node [place] at ($(h2')+(1.4,0)$) (h3')                                              {};
\node  at (h3')  {$a''$};
\node  at ($(h3')+(0.7,0)$)  {$\ldots$};
\node [place] at ($(h3')+(1.4,0)$) (h4')                                              {};
\node [place] at ($(h4')+(0.8,0)$) (h5')                                              {};
\draw ($(h1') + (-0.4,0.6)$) -- ($(h5') + (0.4,0.6)$) -- ($(h5') + (0.4,-0.6)$) -- ($(h1') + (-0.4,-0.6)$) -- cycle;
\node  at ($(h3')+(0,1)$)  {$A''$};

\node [place] (q1') at ($(h1')+(0,-3)$)                                           {};
\node [place] at ($(q1')+(0.8,0)$) (q2')                                              {};
\node  at ($(q2')+(0.7,0)$)  {$\ldots$};
\node [place] at ($(q2')+(1.4,0)$) (q3')                                              {}
edge [thick]                 (h3');

\node  at (q3')  {$c'$};
\node  at ($(q3')+(0.7,0)$)  {$\ldots$};
\node [place] at ($(q3')+(1.4,0)$) (q4')                                              {};
\node [place] at ($(q4')+(0.8,0)$) (q5')                                              {};
\draw ($(q1') + (-0.4,0.6)$) -- ($(q5') + (0.4,0.6)$) -- ($(q5') + (0.4,-0.6)$) -- ($(q1') + (-0.4,-0.6)$) -- cycle;
\node  at ($(q3')+(0,-1)$)  {$C'$};


\path[every node/.style={font=\sffamily\small}]
($(h3') + (0,-1.5)$) edge [dashed, post, bend right=20] node {} ($(w3')+(0,-1.5)$);      

\path[every node/.style={font=\sffamily\small}]
($(h3') + (0,-1.5)$) edge [dashed, pre, bend left=20] node {} ($(w3')+(0,-1.5)$); 

\node[every node/.style={font=\sffamily\small}]  at ($(w3')+(2.7,-1.5)$)  {$\pi$-transformation};
\node  at ($(w5') + (0.55,2.3)$)  {$\overbrace{\hspace{8.6cm}}^{X}$};

\node[every node/.style={font=\sffamily\small}]  at ($(w3')+(2.7,-1.5)$)  {$\pi$-transformation};
\node  at ($(w5') + (0.55,-4.8)$)  {$\underbrace{\hspace{8.6cm}}_{Y}$};
\end{scope}

\draw [-to,thick,snake=snake,segment amplitude=.4mm,
segment length=2mm,line after snake=1mm,color=orange] ($(w1')+(-3,-1)$) -- ($(w1')+(-0.4,-1)$);

\node at ($(w1')+(-1.2,-1.5)$) {$\I$ \hspace{1.5cm} $\cori$};

\begin{pgfonlayer}{background}
\filldraw [line width=4mm,black!07]
($(h5')+(-12.5,3.1)$) rectangle ($(g1')+(-12.5,-2.1)$)
($(h5')+(0.5,3.1)$) rectangle ($(g1')+(-0.5,-2.1)$);
\end{pgfonlayer}

\draw [line width=0.2mm,join=round,black]
($(h5')+(-12.23,3.37)$) rectangle ($(g1')+(-12.77,-2.37)$)
($(h5')+(0.77,3.37)$) rectangle ($(g1')+(-0.77,-2.37)$);

\end{tikzpicture}\caption{The picture on the left shows an instance $\I$ of the maximum 3-dimensional matching problem and the picture in the right shows the corresponding instance $\cori$ of the \matchingproblem\enspace problem. Solid segments show the edges of the graphs and dashed segments specify the corresponding $\pi$-transformations of the edges.}\label{reduction1}
%\end{minipage}
\end{figure}

==> sources/approximation.tex <==
\section{Discretization and Approximation}\label{sec:discretization}
In this section, we show that if the number of pure strategies of the leader is polynomial, one can find an approximation solution for the Stackelberg equilibria of the game by discretizing the mixed strategies of the leader. The running time of the algorithm is regardless of the number of pure strategies of the follower, however as a downside, the accuracy of the solution appears in the exponent of the running time. To this end, we define an approximation solution to the Stackelberg equilibria of a game as follows:

\begin{definition}
	We say a pair of strategies $X_i$ and $Y_i$ of the leader and follower is an $\epsilon$-approximation Stackelberg equilibrium iff
	\begin{itemize}
		\item $Y_i$ is an almost best-response of the follower against $X_i$. More precisely, the payoff of the follower when he plays $Y_i$ against $X_i$ differs by at most $\epsilon$ from the maximum payoff he can get against $X_i$.
		\item The payoff of the leader against $Y_i$ ($\payoffl(X_i,Y_i)$) is at most $\epsilon$ away from the payoff he gets in a Stackelberg equilibrium of the game.
	\end{itemize}
\end{definition}

%In the bilinear setting, every strategy of the players is represented with a vector of some fixed size. We assume w.l.g that the values of these vectors are between $0$ and $1$ (one can shift and scale the values otherwise). The representations should be in a way that the payoffs of the players can be formulated as bilinear functions in terms of the strategy vectors. In other words, for two strategies of the players represented with vectors $X$ and $Y_i$, the payoffs of the players can be formulated as 
%\begin{equation}\label{formula:one}
%\payoffl(X,Y_i) = \sum_i \sum_j \alpha_{i,j} X_i Y_i_j \hspace{1cm} \payofff(X,Y_i) = \sum_i \sum_j \beta_{i,j} X_i Y_i_j
%\end{equation} 
%where $\alpha_{i,j}$'s and $\beta_{i,j}$'s are constant positive coefficients. We refer to the length of the representation vectors as the size of the representation.
We also assume that we have access to an oracle $\phi$ thet optimizes the strategies of the follower over any linear function. In other words, if we represent the strategies of the follower with a vector $Y$, then for any given vector $W$ of the same size, $\phi$ finds us a strategy $Y_i$ of the follower that maximizes $Y_i.W$. For instance, in the case of the matching game, every pure strategy of the follower can be represented with a vector of size $|E(G)|$ whose every element is either $1$, showing the existence of the corresponding edge in the matching of the follower, or $0$ otherwise. As a result, every mixed strategy of the follower is represented by a vector of the same size whose elements have values between $0$ and $1$ which is a mixture of the representations for the corresponding pure strategies. Now, if one wishes to solve  the obave oracle to optimize the strategies of the follower, it only suffices to put the corresponding weights of vector $W$ on the edges of the graph and find  a prefect matching of the graph with the maximum  total weight. Therefore, such an oracle can be implemented in polynomial time.

In what follows we present a discretization method to approximate an SE of a game when the number of strategies of the leader is polynomial and an optimization oracle is provided for the strategies of the follower. The intutition behind the algorithm is to discretize the strategies of the leader. Note that if we were gievn a set of strategies for the leader and were guaranteed  that one element of this set is in fact the strategy of the leader in an SE, then we could iterate over all strategies of this set and verify each strategy by finding its corresponding best-response for the follower. The number of mixed strategies of the leader is infinite and thus iterating over all strategies is impossible. However, one can find a limited number of strategies of the leader and be sure that every strategy of the leader is close to at least one strategy of this set in terms of the distribution of probabilities over the pure strategies. Thus, one strategy of this set is  close to the optimal solution of the leader. Let this strategy be $X_i$ 
and the optimal strategy of the leader in an SE be $\xopt$ and their corresponding best-responses for the follower be $Y_i$ and $\yopt$, respectively. Since $X_i$ and $\xopt$ are close, then the difference between $\payofff(X_i,\yopt)$
	and $\payofff(X_i,Y_i)$ is small. This shows that if instead of focusing on the exact best-responses, we take into account all strategies of the follower against $X_i$ that are almost best-response (best response within an error threshold), $\yopt$ lies in this set. One can then argue that if we find one of such almost best-responses against $X_i$ that maximizes the payoff of the leader, this leads us to an approximation solution.

Based on what mentioned above, the sketch of the algorithm is summarized in the following: Let the number of pure strategies of the leader be $n$. For some $\epsilon > 0$, we construct a set of $O(n^{1/\epsilon})$ strategies of the leader wherein the probabilities of the pure strategies are factors of $\epsilon$. For instance, for $\epsilon = 1/2$, the probability of every pure strategy of the leader can be either  0, $0.5$, or $1$ and that makes a total of $O(n^2)$ mixed strategies. Let this set be $\mathcal{S}$.  We iterate over all strategies $X_i$ of $\mathcal{S}$  and find a best-response for the follower against $X_i$. Let $M$ be the maximum value of the payoff functions for any pair of strategies. For every $X_i$, we first find a strategy $Y_i$ that maximizes $\payofff(X_i,Y_i)$. Then, among all pure strategies $Y^*_i$ of the follower such that $\payofff(X_i,Y_i) - \payofff(X_i,Y^*_i) \leq 2n\epsilon M$ we choose the one that maximizes $\payoffl(X_i,Y^*_i)$ and record this pair as a potential solution. Finally, among all such solutions, we choose the one that maximizes the payoff of the leader and report it as an approximation Staceklberg equilibrium of the game. This proceduce is summerized in Algorithm \ref{alg:discretization}. In the following, we show that this algorithm runs in polynomial time and that indeed finds an approximation SE of the leader.

\begin{algorithm}[h]
	\KwData{Strategies of the leader, $\epsilon$, and an oracle $\phi$ to optimize the strategies of the follower.}
	\KwResult{An approximation SE.}
	$\mathcal{S} \leftarrow$ The set all discretized strategies of the leader\;	
	$\mathsf{Answers} \leftarrow \emptyset$ // This set contains all potential solutions\;
	\For {$X_i \in \mathcal{S}$}{
		$Y_i \leftarrow $ best-response of the follower against $X_i$\;
		$Y^*_i \leftarrow$ the strategy of the follower such that $\payofff(X_i,Y_i) - \payofff(X_i,Y^*_i) \leq 2n\epsilon M$ and $Y^*_i$ maximizes $\payoffl(X_i,Y^*_i)$\;
		Add $(X_, Y^*_i)$ to $\mathsf{Answers}$\;
	}
   Return a solution of $\mathsf{Answers}$ with  the maximum payoff for the leader\;
  	
	\caption{An approximation solution for SE}
		\label{alg:discretization}
\end{algorithm}

\begin{theorem}\label{thm:last}
	For a game with $n$ pure strategies for the leader, given that an optimization oracle is provided for the strategies of the follower, for any $\epsilon > 0$ Algorithm \ref{alg:discretization} runs in polynomial time and finds a $2n\epsilon M$-approximation Stackelberg equilibrium of the game where $M$ is the maximum of the payoffs for any pair of strategies.
\end{theorem}
In the interest of space, we defer the proof of Theorem \ref{thm:last} to the full-version of the paper.
\begin{comment}
\begin{proof}
We first show how one can run Algorithm \ref{alg:discretization} in polynomial time. As mentioned earlier, the size of set $\mathcal{S}$ is bounded by $O(n^{1/\epsilon})$ since for every $\epsilon$ portion of the probability in a mixed strategy, there are at most $n$ choices of pure strategies. Thus, the size of set $\mathcal{S}$ is polynomial in $n$.

For every mixed strategy $X_i$ of set $\mathcal{S}$, we first find a best-response against $X_i$ for the follower. This is possible in polynomial time since the oracle functions are provided. More precisely, we seek to find a pure strategy $Y_i$ of the follower that maximizes $\payofff(X_i,Y_i)$ and since the payoff functions are bilinear, this turns into a linear function over the strategies of the follower and hence one can use the oracle function to find such a best-response in polynomial time. Let the best-response be $Y_i$ and as such, the payoff of the follower for such a strategy be $\payofff(X_i, Y_i)$. Now, we find a strategy $Y^*_i$ that maximizes the payoff of the leader under the follower constraint: The payoff of the follower when playing $Y^*_i$ differs by at most $2n\epsilon M$ from $\payofff(X_i, Y_i)$. This can be done via finding the optimal solution of the following LP.
\begin{eqnarray*}
\max & \payoffl(X_i,Y^*_i)\\
s.t. & \payofff(X_i, Y^*_i) \geq \payofff(X_i, Y_i) - 2n\epsilon M
\end{eqnarray*}
Using Ellipsoid method, the computational complexity of finding such a strategy boils down to optimizing the strategies of the follower that can be done in polynomial time using the optimization oracle~\cite{ahmadinejad2016duels}. Thus, Algorithm \ref{alg:discretization} can be implemented to run in polynomial time.

In what follows, we show that the payoff of the leader in such a solution is at most $2n\epsilon M$ away from that of the optimal Stackelberg equilibrum of the game. Due to the construction of set $\mathcal{S}$, for every mixed strategy $X$, there exists a mixed strategy $X_i$ in set $\mathcal{S}$ such that 
\begin{equation}\label{equation:closeness}
\forall \text{ pure strategy } \hat{x}\hspace{1cm}|\Pr_{x \sim X_i}[x = \hat{x}] - \Pr_{x \sim X}[x = \hat{x}]| \leq \epsilon
\end{equation}
Let the optimal strategy of the leader in a Stackelberg equilibrium be $\xopt$ and a strategy of set $\mathcal{S}$ holding Inequality \eqref{equation:closeness} for $\xopt$ be $X_i$. Similarly, let the best-responses of the follower for strategies $\xopt$ and $X_i$ be $\yopt$ and $Y_i$, respectively. By Inequality \eqref{equation:closeness} we have
\begin{equation}\label{equation:closeness2}
\forall \text{ pure strategy } \hat{x}\hspace{1cm}|\Pr_{x \sim X_i}[x = \hat{x}] - \Pr_{x \sim \xopt}[x = \hat{x}]| \leq \epsilon
\end{equation}
and hence one can argue that $\payofff(\xopt, \yopt) \geq \payofff(\xopt,Y_i) \geq \payofff(X_i,Y_i) - n \epsilon M$. Similarly, $\payofff(X_i,\yopt) \geq \payofff(\xopt,\yopt) - n\epsilon M$ and therefore $\payofff(X_i, \yopt) \geq \payofff(X_i, Y_i) - 2 n \epsilon M$. Hence $\yopt$ lies in the set of mixed strategies whose payoffs against $X_i$ are at most $2n\epsilon M$ away from $\payofff(X_i, Y_i)$. In other words, $\yopt$ is an almost best-response against $X_i$. Notice that by Inequality \eqref{equation:closeness2} we have $\payoffl(X_i, \yopt) \geq \payoffl(\xopt, \yopt) - n\epsilon M$ and thus by maximizing the payoff of the leader among all almost best-responses, the payoff of the leader will be at least $\payoffl(\xopt, \yopt) - n\epsilon M$ which completes the proof.
\end{proof}
\end{comment}

==> sources/apxhardness.tex <==


\section{The \mgame\ Game}\label{section:apx}
%\red{[NH: I made a macro \mgame game that we can use in this section as well.]}
\subsection{Hardness of approximation}
\nhcomment{The first three paragraphs are redundant now that we have the full introduction. I think we should remove it. Add a subsection for hardness of approximation}

%In this section, we discuss the computational complexity of determining the Stackelberg equilibria of huge games. It has been shown that a Stackelberg equilibrium of a game can be found in polynomial time when the follower has polynomially many pure strategies~\cite{paruchuri2008playing}. Note that since the follower always plays a best response in an SE, we can assume w.l.g that the strategy of the follower in an SE is always pure. Therefore, one could iterate over all possible pure strategies of the follower and solve the problem subject to follower's best-response being a fixed pure strategy. To this end, for a fixed pure strategy $Y$ of the follower, we wish to find a strategy $X$ (possibly mixed) of the leader such that (i) $Y$ is a best-response against $X$ and (ii) $X$ maximizes the payoff of the leader against $Y$. Indeed both criteria can be formulated with linear constraints and thus this problem can be modeled with an LP~\cite{paruchuri2008playing}. Thus, an SE of a game can be determined by solving an LP for each pure strategy of the follower and taking the maximum payoff of the leader over all solutions. However, the running time of this solution depends linearly on the number of pure strategies of the follower and thus it does not run in polynomial time when the follower has exponentially many pure strategies.

%Although the problem is trivially intractable when any of the players has exponentially many pure strategies due to the massive input length, it still remains a question whether the problem admits a fast solution for \textit{structured games}. For instance, one could define a game in which players' strategies are the set of all matchings or spanning trees of a graph. As such, the input to the problem is only a graph which is polynomially representable, nonetheless, the players have exponentially many pure strategies. Several recent works aimed at studying the computational complexity of finding an NE of such games~\cite{immorlica2011dueling,ahmadinejad2016duels,behnezhad2016faster,garg2011bilinear,xu2016mysteries,wang2017security}. For instance, the classic approach for computing the equilibria of a two player zero-sum game fails when the players have exponentially many pure strategies. However, \ahmadinejadduels~\cite{ahmadinejad2016duels} prove that it only suffices to be able to optimize a linear function over the strategies of the players in polynomial time to compute the equilibria of a two player zero-sum game in polynomial time. This result holds for all two player zero-sum games regardless of the size of the strategies. Notice that NE and SE are equivalent concepts for zero-sum games~\cite{korzhyk2011stackelberg}, and as such, their result can be seen as a solution for Stackelberg equilibria for the special case of zero-sum games. A natural question that emerges here is whether a similar algorithm can be designed to compute or even approximate an SE of a structured but non-zero-sum game. In what follows, we show that the answer is negative unless P=NP.
The goal of this section is to show a hardness result for the Stackelberg equilibria of large structured games. In contrast to the zero-sum setting, we prove that a polynomial time algorithm for optimizing the strategies in a Stackelberg game does not necessarily lead to a polynomial time solution for Stackelberg equilibria. More precisely, we show that in some cases, the problem of (approximately) computing a Stackelberg equilibrium of a game is NP-hard even if optimization over the strategy space of the players is polynomially tractable.

To this end, we present a game such that any linear function over the strategies of this game can be optimized in polynomial time. Next, we proceed by showing that finding an SE of this game is NP-hard. Moreover, we show that the problem remains hard, even if we wish to approximate an SE of the game within a small error.

We define the \textit{\mgame\  game} as follows: In a \mgame\  game, we have a graph $G$, an injective surjective (one-to-one) function $\pi: E(G) \rightarrow E(G)$ over the edges of $G$ and two players $A$ and $B$. For a set $S$ of the edges of $G$, we define $\pi(S) = \{e \in S| \pi(e)\}$ and assume $\pi(S) = T \Leftrightarrow \pi^{-1}(T) = S$. Note that we assume that $G$ is a multigraph and may contain parallel edges between a pair of vertices. In this case, the $\pi$ values for two parallel edge may differ. In thes rest of this section, every time we use the term graph we refer to a multigraph. Each player's pure strategy is a matching of $G$ and for two matching $M_A$ and $M_B$ for players $A$ and $B$ we define the payoffs of the players as follows:
\begin{equation*}
\payoffa(M_A,M_B) = |M_A \cap \pi(M_B)| \hspace{2cm} \payoffb(M_A,M_B) = |M_A \cap M_B|
\end{equation*} 

\begin{center}
    \noindent\framebox{\begin{minipage}{6.50in}
            \textsf{\mgame\ }\\[0.25cm]
            \textsf{Input}: An unweighted undirected graph $G$ and an injective surjective function $\pi$ over the edges of $G$. \\[0.25cm]
            \textsf{Players strategies:} Each players pure strategies is the set of all matchings of $G$.\\[0.25cm]
            \textsf{Player $A$'s payoff:} The number of edges his matching has in common with the $\pi$-transformation of player $B$'s matching.\\[0.25cm]
            \textsf{Player $B$'s payoff:} The number of edges his matching has in common with player $A$'s matching.\\[0.25cm]
    \end{minipage}}
\end{center}

Note that $G$ and $\pi$ are known to both players in advance. We refer to player $A$ as leader and call player $B$ the follower. Each strategy of the players in this game can be represented with a 0-1 vector of size $|E(G)|$ whose every element specifies whether a particular edge appears in the matching. We first show that the strategies of both players can be optimized with respect to any linear function over the edges of the graph.


%\red{[NH: Add the zero-sum version of the results in a theorem environment.]}

\begin{observation}\label{salam1}
    There exists a polynomial time algorithm such that for every vector $w$ of size $|E(G)|$ finds a strategy of the players whose corresponding representation vector $v$ maximizes $v.w$.
\end{observation}
\begin{proof}
    This problem reduces to finding a maximum weighted matching of a graph. We associate a weight $w_e$ to every edge $e$ of the graph which is equal to the value of the corresponding element of $e$ in vector $w$. Now, the weight of any matching in this graph is equal to the dot product of $w$ and the representation vector of the matching and thus the problem reduces to finding the maximum weighted matching of the graph which can be done in polynomial time ~\cite{cormen2009introduction}.
\end{proof}

Recall that Observation \ref{salam1} is enough for the framework of \ahmadinejadduels~\cite{ahmadinejad2016duels} to show that an NE (or equivalently an SE) of the game can be computed in polynomial time for a zero-sum variant of the game. However, as we show, this property alone does not guarantee a polynomial time solution for the case of Stackelberg equilibria of non-zero-sum games.
In what follows we show that it is impossible to approximate a Stackelberg equilibrium of the \mgame\  game in polynomial time within an arbitrarily small constant factor unless P=NP.

Before we proceed to the proof, we define an auxiliary problem and show a hardness result for this problem. Later we take advantage of this hardness result to show an APX-hardness result for finding a Stackelberg equilibrium of the \mgame\  game. To this end, we define \textit{the \matchingproblem\enspace problem} as follows:

\begin{center}
    \noindent\framebox{\begin{minipage}{6.50in}
            \textsf{\matchingproblem\enspace}\\[0.25cm]
            \textsf{Input}: An unweighted undirected graph $G$ and an injective surjective function $\pi: E(G) \rightarrow E(G)$ over the edges of $G$. \\[0.25cm]
            \textsf{Output:} A matching $M$ of $G$ such that $|M \cap \pi(M)|$ is maximized.\\[0.25cm]
    \end{minipage}}
\end{center}

We show that \matchingproblem\enspace has a \textit{hard gap} at \textit{gap location $1$}. In other words, it is NP-hard to decide whether for a given graph $G$ with $n$ vertices and a function $\pi$, the solution of the \matchingproblem\enspace problem is exactly equal to $n/2$ or at most $(1-\epsilon)n/2$ for some $\epsilon > 0$.

\begin{lemma}\label{lm1}
    There exists an $\epsilon > 0$ such that it is NP-hard to decide whether the solution of the \matchingproblem\enspace problem is exactly equal to $n/2$ or less than $(1-\epsilon)n/2$ where $n$ is the number of the vertices of the input graph.
\end{lemma}
Another way to phrase Lemma \ref{lm1} is that the \matchingproblem\enspace problem has a hard gap at gap location 1. For brevity, we skip the proof of Lemma \ref{lm1} here and defer it to the end of this section. Based on Lemma \ref{lm1}, we are now ready to prove the main result of this section.

\begin{theorem}\label{apxhardness} \label{thm:apxhardness}
    Computing a Stackelberg equilibrium of the \mgame\  game is APX-hard.
\end{theorem}
\begin{proof}
    More generally we show that approximating a Stackelberg equilibrium of the \mgame\  game has a hard gap at gap location $1$. This immediately implies a hardness of approximation. We show this by a reduction from the \matchingproblem\enspace problem. Suppose we are given an instance $\I = \langle G, \pi\rangle$ of the \matchingproblem\enspace problem and wish to decide for some $\epsilon' > 0$, whether the solution of this problem is exactly $n/2$ or it is bounded by $(1-\epsilon')n/2$ where $n$ is the size of $G$.
    Based on $\I$, we construct an instance $\cori$ of the \mgame\  game with the same graph $G$ and transformation function $\pi$ and seek to find a Stackelberg equilibrium of the leader (player $A$) in this game. Note that by definition, the solution of $\I$ is equal to $n/2$ if and only if $G$ contains a perfect matching which is identical to its $\pi$-transformation. Otherwise, the solution of $\I$ is at most $(1-\epsilon')n/2$ and thus any matching of $G$ shares no more than $(1-\epsilon')n/2$ edges with its $\pi$-transformation.
    
    Since for small enough $\epsilon'$ it is NP-hard to distinguish the two cases (Lemma \ref{lm1}), we show that it is NP-hard to approximate a Stackelberg equilibrium of the leader in $\cori$. If the solution of $\I$ is $n/2$, then there exists a perfect matching in $G$ which is identical to its $\pi$-transformation. Thus, if both players play this matching in $\cori$, they both get a payoff of $n/2$ and since $n/2$ is the maximum possible payoff for any player in this game, this makes the game a Stackelberg equilibrium for the leader. Therefore, in this case, the leader achieves a payoff of $n/2$ in a Stackelberg equilibrium of the \mgame\  game. 
    
    Now, suppose for $\epsilon < \epsilon'/13$ we have a $1-\epsilon$ approximation solution for $\cori$. If the solution of $\I$ is $n/2$, then the payoff of the leader in such an approximation solution is at least $n(1-\epsilon)/2$. Let the strategies of the leader and follower be $X$ and $Y$ in this solution. Therefore, $\payoffa(X,Y) \geq n(1-\epsilon)/2$. Notice that $X$ may be a mixed strategy, but we can assume w.l.g that $Y$ is a pure strategy since there always exists a best response for the follower which is pure. Also, let $Y^*$ be the $\pi$-transformation of strategy $Y$. Let for two matchings $x$ and $y$, $\common(x,y)$ denote the number of edges that $x$ and $y$ have in common and define $\dist(x,y) = |x| + |y|-2\common(x,y)$. Recall that the payoff of player $A$ in this game can be formulated as $\mathbb{E}_{x \sim X} [\common(x,Y^*)]$. Since this value is at least $n(1-\epsilon)/2$ we have:
    \begin{equation*}
    \mathbb{E}_{x \sim X} [\common(x,Y^*)] = \payoffa(X,Y) \geq n(1-\epsilon)/2
    \end{equation*}
    and thus
    \begin{equation}\label{fact1}
    \begin{split}
    \mathbb{E}_{x \sim X} [\dist(x,Y^*)] & =  \mathbb{E}_{x \sim X} [|x| + |Y^*| - 2\common(x,Y^*)]\\
    & \leq  \mathbb{E}_{x \sim X} [n - 2\common(x,Y^*)]\\
    & = n - 2\mathbb{E}_{x \sim X} [\common(x,Y^*)]\\
    & \leq n - 2 n(1-\epsilon)/2\\
    & = n - n(1-\epsilon)\\
    & \leq n \epsilon.
    \end{split}
    \end{equation}
    Inequality \eqref{fact1} shows that $Y^*$ is very similar (in expectation) to a random matching drawn from strategy $X$. This intuitively implies that pure strategies of $X$ should have lots of edges in common. It follows from the definition that for three matchings $x$, $y$, and $z$ we have $\dist(x,z) \leq \dist(x,y) + \dist(y,z)$. Therefore, we have 
    \begin{equation}\label{fact2}
    \begin{split}
    \mathbb{E}_{x \sim X, x' \sim X} [\dist(x,x')] & \leq \mathbb{E}_{x \sim X, x' \sim X} [\dist(x,Y^*) + \dist(Y^*,x')]\\
    & = \mathbb{E}_{x \sim X, x' \sim X} [\dist(x,Y^*) + \dist(x', Y^*)]\\
    & = \mathbb{E}_{x \sim X} [\dist(x,Y^*)] + \mathbb{E}_{x' \sim X} [\dist(x',Y^*)]\\
    & = 2 \mathbb{E}_{x \sim X} [\dist(x,Y^*)]\\
    & \leq 2\epsilon n
    \end{split}
    \end{equation}
    Recall that the payoff of the follower is determined by the number of edges his matching shares with that of the leader. Recall that since $\payoffa(X,Y) \geq n(1-\epsilon)/2$, this implies that $\mathbb{E}_{x \sim X}[|x|] \geq n(1-\epsilon)/2$. What Inequality \eqref{fact2} implies is that if the follower plays $X$ instead of $Y$, he gets a payoff of at least $\mathbb{E}_{x \sim X}|x| - 2\epsilon n \geq (1-5\epsilon)n/2$ against $X$. In other words $\payoffb(X,X) \geq (1-5\epsilon)n/2$. Since $Y$ is a best response of the follower against the leader's strategy, we have $\payoffb(X,Y) \geq \payoffb(X,X) \geq (1-5\epsilon)n/2$ and thus
    \begin{equation*}
    \begin{split}
    \mathbb{E}_{x \sim X} [\common(x,Y)] & = \payoffb(X,Y) \\
    & \geq \payoffb(X,X)\\
    & =  \mathbb{E}_{x \sim X, x' \sim X} [\common(x,x')]\\
    & \geq (1-5\epsilon)n/2.
    \end{split}
    \end{equation*}
    Hence
    \begin{equation}\label{fact3}
    \begin{split}
    \mathbb{E}_{x \sim X} [\dist(x,Y)] & = \mathbb{E}_{x \sim X} [|x| + |Y| - 2\common(x,Y)] \\
    & \leq \mathbb{E}_{x \sim X} [n - 2\common(x,Y)]\\
    & = n-2\mathbb{E}_{x \sim X} [\common(x,Y)]\\
    & \leq n-2(1-5\epsilon)n/2\\
    & \leq 5\epsilon n
    \end{split}
    \end{equation}
    Combining Inequalities \eqref{fact1} and \eqref{fact3} yields
    \begin{equation*}
    \dist(Y, Y^*) \leq \mathbb{E}_{x \sim X} [\dist(x,Y)] + \mathbb{E}_{x \sim X} [\dist(x,Y^*)] \leq 6\epsilon n.
    \end{equation*}
    Therefore, we have $\common(Y, Y^*) \geq |Y^*|- 6\epsilon n$ and since $|Y^*| \geq (1-\epsilon)n/2$ we have $\common(Y, Y^*) \geq (1-13\epsilon)n/2  >  (1-\epsilon')n/2$. Now, if the solution of $\I$ is not $n/2$, then it is at most $(1-\epsilon')n/2$. Therefore, $\common(Y, Y^*) > (1-\epsilon')n/2$ happens if and only if the solution of $I$ is exactly $n/2$. Thus, an approximation solution for $\cori$ within a factor $(1-\epsilon) > (1-\epsilon'/13)$ can be used to decide if the solution of $\I$ is $n/2$ or bounded by $(1-\epsilon')n/2$. This implies a hard gap for the \matchingproblem\enspace problem at gap location $1$.
\end{proof}

All that remains is to prove the statement of Lemma \ref{lm1} and that completes the proof Theorem \ref{apxhardness}.

\begin{proof}[of Lemma \ref{lm1}]
    \input{figs/reduction1.tex}
    We show this lemma by a reduction from the \threedM\enspace problem. In \threedM\enspace problem, we are given a hypergraph $G$ whose vertices are divided into three parts $A$, $B$, and $C$. Every edge of $G$ is a triple $(a,b,c)$ of the vertices such that $a \in A$, $b \in B$, and $c \in C$ hold. A matching in this graph is a subset of the edges that do not share any vertices. The goal of the problem is to find a matching with the maximum number of edges. \petrankhardness~\cite{petrank1994hardness} showed that the \threedM\enspace problem has a hard gap at gap location $1$.
    
    We show via a reduction that \matchingproblem\enspace is harder than the \threedM\enspace problem. This implies a similar hardness result for the \matchingproblem\enspace problem. To this end, suppose we are given an instance $\I$ of the 3-dimensional matching problem. Let the graph of this instance be $G$ and its vertices lie in three parts $A$, $B$, and $C$ such that every edge of the graph contains a vertex of each part. We construct a bipartite graph $G'$ and a function $\pi$ based on $G$ as follows:
    \begin{itemize}
        \item $G'$ contains two independent parts $X$ and $Y$, each of which contains an endpoint of every edge of the graph.
        \item $X = A' \cup A''$ where  $A'$ and $A''$ are two copies of $A$.
        \item $Y = B' \cup C'$ where $B'$ is a copy of $B$ and $C'$ is a copy of $C$.
        \item For every vertex $a \in A$, we put two vertices $a'$ and $a''$ in $X$ (in $A'$ and $A''$ respectively).
        \item For every vertex $b \in B$ we put a vertex $b'$ in $Y$ (in part $B'$).
        \item For every vertex $c \in C$ we put a vertex $c'$ in $Y$ (in part $C'$).
        \item For every edge $(a,b,c)$ of $G$, we put two edges $(a',b')$ and $(a'',c')$ in $G'$. Moreover, we set $\pi((a',b')) = (a'',c')$ and $\pi((a'',c')) = (a',b')$. Note that this way, there may be multiple edges between two vertices of $G$ with different $\pi$ values.
    \end{itemize}
    Now, we argue that for every 3-dimensional matching $M$ of $G$, there exists a matching $M'$ of $G'$ such that $|M' \cap \pi(M')| = 2|M|$ and viceversa. To this end, suppose $M$ is a 3-dimensional matching of $G$. Now, we set $M' = \{(a,b,c) \in E(G) | (a',b')\} \cup \{(a,b,c) \in E(G) | (a'',c')\}$. Since $M$ is a matching, no two edges of $M'$ share a vertex and thus $M'$ is also a matching. Moreover, for every edge in $M'$, its $\pi$ transformation is also included in $M'$ and therefore $M' = \pi(M')$. Hence $|M' \cap \pi(M')| = |M'| = 2|M|$. A similar argument shows that for any matching $M'$ of $G'$ such that $|M' \cap \pi(M')| = 2k$, there exists a matching of size $k$ in $G$. Therefore, the problem of finding a maximum 3-dimensional matching of $G$ reduces to finding a matching of $G'$ that shares the maximum number of edges with its $\pi$-transformation. Since \threedM\enspace problem has a hard gap at gap location $1$, so does the \matchingproblem\enspace problem. Figure \ref{reduction1} describes the reduction mentioned above.
\end{proof}
\subsection{A $1/12$ Approximation Solution}
In Section \ref{section:apx}, we showed that approximating an SE of the \mgame\  game within an arbitrarily small error is NP-hard. We complement this result by presenting a polynomial time algorithm to compute a $1/12$-approximation solution. In other words, our algorithm provides a strategy $X$ for the leader that achieves at least a $1/12$ fraction of the payoff of an SE against the best response of his opponent.

We first devise a greedy algorithm to find two matchings $x$ and $x'$ such that $x$ shares as many edges as possible with the $\pi$-transformation of $x'$. To this end, we begin with two empty matchings $x$ and $x'$ and every time choose two edges $e$ and $e'$ of the graph such that $\pi(e') = e$, $e$ is not adjacent\footnote{two edges are adjacent if they share a common vertex.} to any edge of $x$, and $e'$ is not adjacent to any edge of $x'$. Next, we update the matchings by adding $e$ to $x$ and $e'$ to $x'$.

\begin{algorithm}
    \label{alg:matchings}
    \KwData{A graph $G$ and a one-to-one mapping $\pi$ over the edges of $G$.}
    \KwResult{Two matchings $x$ and $x'$.}
    $x \leftarrow \emptyset$\;    
    $x' \leftarrow \emptyset$\;
    \While{\text{there exist edges $e$ and $e'$ s.t} \begin{itemize}
                \item $e = \pi(e')$
                \item \text{$e$ doesn't share any vertices with $x$}
                \item \text{$e'$ doesn't share any vertices with $x'$}
            \end{itemize}}{
            \text{Add $e$ to $x$}\;
            \text{Add $e'$ to $x'$}\;
    }
    \textbf{Return}$(x,x')$\;
    \caption{Maximizing the number of edges that $x$ shares with $\pi(x')$}
\end{algorithm}

We show that Algorithm \ref{alg:matchings} obtains a $1/4$ approximation solution. Let $x$ and $x'$ be the matchings provided by Algorithm \ref{alg:matchings} and suppose for the sake of contradiction that there exist two matchnigs $y$ and $y'$ such that $\common(y,\pi(y')) > 4\common(x,\pi(x'))$. Due to Algorithm \ref{alg:matchings}, we have $|x| = |x'| = \common(x,\pi(x'))$. Moreover, there are at least $4\common(x,\pi(x'))$ edges in $y'$ whose $\pi$-transformations appear in $y$. Notice that for every edge $e'$ in $x'$, there are at most four of such edges in $y'$ such that either share an end-point with $e'$ or their $\pi$-transformations share an endpoint with $\pi(e')$. Thus, there exists an edge $e'$ in $y$ such that neither $e'$ shares a vertex with the vertices of $x'$ nor $\pi(e')$ shares an endpoint with the vertices of $x$. This is a contradiction since our algorithm terminates when no such pair of edges exists. This observation implies that $|x \cap \pi(x')|$ is at least $1/4$ fraction of the payoff of the leader in any SE.

\begin{observation}\label{observation:matchings}
    Let $x$ and $x'$ be the matchings determined by Algorithm \ref{alg:matchings}. $|x \cap \pi(x')|$ is at least $1/4$ fraction of the optimal payoff the leader gets in an SE.
\end{observation}
\begin{proof}
    Recall that the payoff of the leader is the number of edges his matching has in common with the $\pi$-transformation of the follower's matching. This value is always upper bounded by $4|x \cap \pi(x')|$ for any pair of matchings and thus the proof is complete.
\end{proof}

Let $\epsilon > 0$ be an arbitrarily small positive number and $X$ be a strategy of the leader that plays matching $x$ with probability $1/3-\epsilon$ and matching $x'$ with probability $2/3+\epsilon$. Moreover, let $Y$ be a best response of the follower against $X$. Based on Observation \ref{observation:matchings}, we show that $\payoffa(X,Y)$ is at least $(1-3\epsilon)/12$ fractional of the optimal payoff the leader can get in any SE.

\begin{theorem}
    Let $X$ and $Y$ be the strategies of the leader and the follower defined above. $\payoffa(X,Y)$ is at least $(1-3\epsilon)/12$ fraction of the optimal payoff the leader achieves in any SE.
\end{theorem}
\begin{proof}
    We assume w.l.g that $Y$ is a pure strategy. We first show that $Y$ contains all edges of $x'$. To this end, suppose for the sake of contradiction that an edge $e'$ of $x'$ doesn't appear in $Y$. If we add this edge to $Y$ and remove the edges of $Y$ that share an endpoint with $e'$ then the payoff of the follower changes as follows: Because $X$ plays $x'$ with probability $2/3+\epsilon$ then  $e'$ appears in his strategy with probability $2/3+\epsilon$ and thus the payoff of the follower is increased by $2/3+\epsilon$. Moreover, none of the crossing edges of $e'$ with edges of $Y$ are in $x'$ and thus appear in the leader's strategy with probability at most $1/3-\epsilon$. This incurs a loss of at most $2(1/3-\epsilon) < 2/3+\epsilon$. Thus, this change improves the payoff of the follower which shows $Y$ is not a best response against $X$ which is a contradiction.
    
    Note that $X$ plays $x$ with probability $1/3-\epsilon$ and $Y$ contains every edge of $x'$. Thus, the payoff of the leader is at least $$(1/3-\epsilon)\payoffa(x,x') = (1/3-\epsilon) \common(x,\pi(x')) = (1-3\epsilon) \common(x,\pi(x'))/3.$$ This along with the fact that the payoff of the leader in any SE is at most $4\common(x,\pi(x'))$ (Observation \ref{observation:matchings}) proves that $\payoffa(x,y)$ is at least a $(1-3\epsilon)/12$ fraction of the optimal payoff the leader achieves in any SE.
\end{proof}

==> sources/apxhardness_backup.tex <==


\section{The \mgame\ Game}\label{section:apx}

\nhedit{In this section, we introduce a large but structured Stackelberg game, \mgame, and examine the computational complexity of computing its Stackelberg equilibrium. We show two sets of results for this game. In Section~\ref{section:apx}, we show the existing structure in \mgame is not sufficient for efficient computation of  Stackelberg equilibrium  -- we show that this problem is APX-hard. In Section~\ref{sec:mgame-approx}, we give an efficient $\frac 12$ approximation.

Here, let us highlight an important aspect of our hardness results in advance. As we will show, the strategy space of the players in \mgame Game, though large, is very structured. At a high level, the reward of each player is a linear function of the action of the other and each player can optimize a linear function over the strategy of the other player, for example, each player can compute a best-response  to a mixed strategy of the other. In a zero-sum game, existence of such a structure leads to efficient algorithms for computing the Nash or Stackelberg equilibria~\cite{ahmadinejad2016duels, DHL+17, KV05}. On the other hand, our APX-hardness result for the \mgame game shows that existence of this structure does not necessarily lead to efficient algorithms for computing Stackelberg equilibira in general-sum games. 

With this in mind, let us describe the \mgame games as follows. Consider a multigraph $G$, a one-to-one mapping $\pi: E(G) \rightarrow E(G)$ over the edges of $G$ and two players $A$ and $B$ taking the roles of the leader and follower, respectively.
For a set $S$ of the edges of $G$, we define $\pi(S) = \{e \in S| \pi(e)\}$ and assume $\pi(S) = T \Leftrightarrow \pi^{-1}(T) = S$. Note that we assume that $G$ is a multigraph and may contain parallel edges between a pair of vertices. In this case, the $\pi$ values for two parallel edge may differ. In thes rest of this section, every time we use the term graph we refer to a multigraph. Each player's pure strategy is a matching of $G$ and for two matching $M_A$ and $M_B$ for players $A$ and $B$ we define the payoffs of the players as follows:
\begin{equation*}
\payoffa(M_A,M_B) = |M_A \cap \pi(M_B)| \hspace{2cm} \payoffb(M_A,M_B) = |M_A \cap M_B|
\end{equation*} 

Note that $G$ and $\pi$ are known to both players in advance. We refer to player $A$ as leader and call player $B$ the follower.

}

\subsection{Hardness of approximation}
%\nhcomment{The first three paragraphs are redundant now that we have the full introduction. I think we should remove it. Add a subsection for hardness of approximation}

%In this section, we discuss the computational complexity of determining the Stackelberg equilibria of huge games. It has been shown that a Stackelberg equilibrium of a game can be found in polynomial time when the follower has polynomially many pure strategies~\cite{paruchuri2008playing}. Note that since the follower always plays a best response in an SE, we can assume w.l.g that the strategy of the follower in an SE is always pure. Therefore, one could iterate over all possible pure strategies of the follower and solve the problem subject to follower's best-response being a fixed pure strategy. To this end, for a fixed pure strategy $Y$ of the follower, we wish to find a strategy $X$ (possibly mixed) of the leader such that (i) $Y$ is a best-response against $X$ and (ii) $X$ maximizes the payoff of the leader against $Y$. Indeed both criteria can be formulated with linear constraints and thus this problem can be modeled with an LP~\cite{paruchuri2008playing}. Thus, an SE of a game can be determined by solving an LP for each pure strategy of the follower and taking the maximum payoff of the leader over all solutions. However, the running time of this solution depends linearly on the number of pure strategies of the follower and thus it does not run in polynomial time when the follower has exponentially many pure strategies.

%Although the problem is trivially intractable when any of the players has exponentially many pure strategies due to the massive input length, it still remains a question whether the problem admits a fast solution for \textit{structured games}. For instance, one could define a game in which players' strategies are the set of all matchings or spanning trees of a graph. As such, the input to the problem is only a graph which is polynomially representable, nonetheless, the players have exponentially many pure strategies. Several recent works aimed at studying the computational complexity of finding an NE of such games~\cite{immorlica2011dueling,ahmadinejad2016duels,behnezhad2016faster,garg2011bilinear,xu2016mysteries,wang2017security}. For instance, the classic approach for computing the equilibria of a two player zero-sum game fails when the players have exponentially many pure strategies. However, \ahmadinejadduels~\cite{ahmadinejad2016duels} prove that it only suffices to be able to optimize a linear function over the strategies of the players in polynomial time to compute the equilibria of a two player zero-sum game in polynomial time. This result holds for all two player zero-sum games regardless of the size of the strategies. Notice that NE and SE are equivalent concepts for zero-sum games~\cite{korzhyk2011stackelberg}, and as such, their result can be seen as a solution for Stackelberg equilibria for the special case of zero-sum games. A natural question that emerges here is whether a similar algorithm can be designed to compute or even approximate an SE of a structured but non-zero-sum game. In what follows, we show that the answer is negative unless P=NP.


The goal of this section is to show a hardness result for the Stackelberg equilibria of large structured games. In contrast to the zero-sum setting, we prove that a polynomial time algorithm for optimizing the strategies in a Stackelberg game does not necessarily lead to a polynomial time solution for Stackelberg equilibria. More precisely, we show that in some cases, the problem of (approximately) computing a Stackelberg equilibrium of a game is NP-hard even if optimization over the strategy space of the players is polynomially tractable.

To this end, we present a game such that any linear function over the strategies of this game can be optimized in polynomial time. Next, we proceed by showing that finding an SE of this game is NP-hard. Moreover, we show that the problem remains hard, even if we wish to approximate an SE of the game within a small error.


%We define the \textit{\mgame\  game} as follows: In a \mgame\  game, we have a graph $G$, an injective surjective (one-to-one) function $\pi: E(G) \rightarrow E(G)$ over the edges of $G$ and two players $A$ and $B$. For a set $S$ of the edges of $G$, we define $\pi(S) = \{e \in S| \pi(e)\}$ and assume $\pi(S) = T \Leftrightarrow \pi^{-1}(T) = S$. Note that we assume that $G$ is a multigraph and may contain parallel edges between a pair of vertices. In this case, the $\pi$ values for two parallel edge may differ. In thes rest of this section, every time we use the term graph we refer to a multigraph. Each player's pure strategy is a matching of $G$ and for two matching $M_A$ and $M_B$ for players $A$ and $B$ we define the payoffs of the players as follows:
%\begin{equation*}
%\payoffa(M_A,M_B) = |M_A \cap \pi(M_B)| \hspace{2cm} \payoffb(M_A,M_B) = |M_A \cap M_B|
%\end{equation*} 

%\begin{center}
%    \noindent\framebox{\begin{minipage}{6.50in}
%            \textsf{\mgame\ }\\[0.25cm]
%            \textsf{Input}: An unweighted undirected graph $G$ and an injective surjective function $\pi$ over the edges of $G$. \\[0.25cm]
%            \textsf{Players strategies:} Each players pure strategies is the set of all matchings of $G$.\\[0.25cm]
%            \textsf{Player $A$'s payoff:} The number of edges his matching has in common with the $\pi$-transformation of player $B$'s matching.\\[0.25cm]
%            \textsf{Player $B$'s payoff:} The number of edges his matching has in common with player $A$'s matching.\\[0.25cm]
%    \end{minipage}}
%\end{center}

Note that $G$ and $\pi$ are known to both players in advance. We refer to player $A$ as leader and call player $B$ the follower. Each strategy of the players in this game can be represented with a 0-1 vector of size $|E(G)|$ whose every element specifies whether a particular edge appears in the matching. We first show that the strategies of both players can be optimized with respect to any linear function over the edges of the graph.


%\red{[NH: Add the zero-sum version of the results in a theorem environment.]}

\begin{observation}\label{salam1}
    There exists a polynomial time algorithm such that for every vector $w$ of size $|E(G)|$ finds a strategy of the players whose corresponding representation vector $v$ maximizes $v.w$.
\end{observation}
\begin{proof}
    This problem reduces to finding a maximum weighted matching of a graph. We associate a weight $w_e$ to every edge $e$ of the graph which is equal to the value of the corresponding element of $e$ in vector $w$. Now, the weight of any matching in this graph is equal to the dot product of $w$ and the representation vector of the matching and thus the problem reduces to finding the maximum weighted matching of the graph which can be done in polynomial time ~\cite{cormen2009introduction}.
\end{proof}

Recall that Observation \ref{salam1} is enough for the framework of \ahmadinejadduels~\cite{ahmadinejad2016duels} to show that an NE (or equivalently an SE) of the game can be computed in polynomial time for a zero-sum variant of the game. However, as we show, this property alone does not guarantee a polynomial time solution for the case of Stackelberg equilibria of non-zero-sum games.
In what follows we show that it is impossible to approximate a Stackelberg equilibrium of the \mgame\  game in polynomial time within an arbitrarily small constant factor unless P=NP.

Before we proceed to the proof, we define an auxiliary problem and show a hardness result for this problem. Later we take advantage of this hardness result to show an APX-hardness result for finding a Stackelberg equilibrium of the \mgame\  game. To this end, we define \textit{the \matchingproblem\enspace problem} as follows:

\begin{center}
    \noindent\framebox{\begin{minipage}{6.50in}
            \textsf{\matchingproblem\enspace}\\[0.25cm]
            \textsf{Input}: An unweighted undirected graph $G$ and an injective surjective function $\pi: E(G) \rightarrow E(G)$ over the edges of $G$. \\[0.25cm]
            \textsf{Output:} A matching $M$ of $G$ such that $|M \cap \pi(M)|$ is maximized.\\[0.25cm]
    \end{minipage}}
\end{center}

We show that \matchingproblem\enspace has a \textit{hard gap} at \textit{gap location $1$}. In other words, it is NP-hard to decide whether for a given graph $G$ with $n$ vertices and a function $\pi$, the solution of the \matchingproblem\enspace problem is exactly equal to $n/2$ or at most $(1-\epsilon)n/2$ for some $\epsilon > 0$.

\begin{lemma}\label{lm1}
    There exists an $\epsilon > 0$ such that it is NP-hard to decide whether the solution of the \matchingproblem\enspace problem is exactly equal to $n/2$ or less than $(1-\epsilon)n/2$ where $n$ is the number of the vertices of the input graph.
\end{lemma}
Another way to phrase Lemma \ref{lm1} is that the \matchingproblem\enspace problem has a hard gap at gap location 1. For brevity, we skip the proof of Lemma \ref{lm1} here and defer it to the end of this section. Based on Lemma \ref{lm1}, we are now ready to prove the main result of this section.

\begin{theorem}\label{apxhardness} \label{thm:apxhardness}
    Computing a Stackelberg equilibrium of the \mgame\  game is APX-hard.
\end{theorem}
\begin{proof}
    More generally we show that approximating a Stackelberg equilibrium of the \mgame\  game has a hard gap at gap location $1$. This immediately implies a hardness of approximation. We show this by a reduction from the \matchingproblem\enspace problem. Suppose we are given an instance $\I = \langle G, \pi\rangle$ of the \matchingproblem\enspace problem and wish to decide for some $\epsilon' > 0$, whether the solution of this problem is exactly $n/2$ or it is bounded by $(1-\epsilon')n/2$ where $n$ is the size of $G$.
    Based on $\I$, we construct an instance $\cori$ of the \mgame\  game with the same graph $G$ and transformation function $\pi$ and seek to find a Stackelberg equilibrium of the leader (player $A$) in this game. Note that by definition, the solution of $\I$ is equal to $n/2$ if and only if $G$ contains a perfect matching which is identical to its $\pi$-transformation. Otherwise, the solution of $\I$ is at most $(1-\epsilon')n/2$ and thus any matching of $G$ shares no more than $(1-\epsilon')n/2$ edges with its $\pi$-transformation.
    
    Since for small enough $\epsilon'$ it is NP-hard to distinguish the two cases (Lemma \ref{lm1}), we show that it is NP-hard to approximate a Stackelberg equilibrium of the leader in $\cori$. If the solution of $\I$ is $n/2$, then there exists a perfect matching in $G$ which is identical to its $\pi$-transformation. Thus, if both players play this matching in $\cori$, they both get a payoff of $n/2$ and since $n/2$ is the maximum possible payoff for any player in this game, this makes the game a Stackelberg equilibrium for the leader. Therefore, in this case, the leader achieves a payoff of $n/2$ in a Stackelberg equilibrium of the \mgame\  game. 
    
    Now, suppose for $\epsilon < \epsilon'/13$ we have a $1-\epsilon$ approximation solution for $\cori$. If the solution of $\I$ is $n/2$, then the payoff of the leader in such an approximation solution is at least $n(1-\epsilon)/2$. Let the strategies of the leader and follower be $X$ and $Y$ in this solution. Therefore, $\payoffa(X,Y) \geq n(1-\epsilon)/2$. Notice that $X$ may be a mixed strategy, but we can assume w.l.g that $Y$ is a pure strategy since there always exists a best response for the follower which is pure. Also, let $Y^*$ be the $\pi$-transformation of strategy $Y$. Let for two matchings $x$ and $y$, $\common(x,y)$ denote the number of edges that $x$ and $y$ have in common and define $\dist(x,y) = |x| + |y|-2\common(x,y)$. Recall that the payoff of player $A$ in this game can be formulated as $\mathbb{E}_{x \sim X} [\common(x,Y^*)]$. Since this value is at least $n(1-\epsilon)/2$ we have:
    \begin{equation*}
    \mathbb{E}_{x \sim X} [\common(x,Y^*)] = \payoffa(X,Y) \geq n(1-\epsilon)/2
    \end{equation*}
    and thus
    \begin{equation}\label{fact1}
    \begin{split}
    \mathbb{E}_{x \sim X} [\dist(x,Y^*)] & =  \mathbb{E}_{x \sim X} [|x| + |Y^*| - 2\common(x,Y^*)]\\
    & \leq  \mathbb{E}_{x \sim X} [n - 2\common(x,Y^*)]\\
    & = n - 2\mathbb{E}_{x \sim X} [\common(x,Y^*)]\\
    & \leq n - 2 n(1-\epsilon)/2\\
    & = n - n(1-\epsilon)\\
    & \leq n \epsilon.
    \end{split}
    \end{equation}
    Inequality \eqref{fact1} shows that $Y^*$ is very similar (in expectation) to a random matching drawn from strategy $X$. This intuitively implies that pure strategies of $X$ should have lots of edges in common. It follows from the definition that for three matchings $x$, $y$, and $z$ we have $\dist(x,z) \leq \dist(x,y) + \dist(y,z)$. Therefore, we have 
    \begin{equation}\label{fact2}
    \begin{split}
    \mathbb{E}_{x \sim X, x' \sim X} [\dist(x,x')] & \leq \mathbb{E}_{x \sim X, x' \sim X} [\dist(x,Y^*) + \dist(Y^*,x')]\\
    & = \mathbb{E}_{x \sim X, x' \sim X} [\dist(x,Y^*) + \dist(x', Y^*)]\\
    & = \mathbb{E}_{x \sim X} [\dist(x,Y^*)] + \mathbb{E}_{x' \sim X} [\dist(x',Y^*)]\\
    & = 2 \mathbb{E}_{x \sim X} [\dist(x,Y^*)]\\
    & \leq 2\epsilon n
    \end{split}
    \end{equation}
    Recall that the payoff of the follower is determined by the number of edges his matching shares with that of the leader. Recall that since $\payoffa(X,Y) \geq n(1-\epsilon)/2$, this implies that $\mathbb{E}_{x \sim X}[|x|] \geq n(1-\epsilon)/2$. What Inequality \eqref{fact2} implies is that if the follower plays $X$ instead of $Y$, he gets a payoff of at least $\mathbb{E}_{x \sim X}|x| - 2\epsilon n \geq (1-5\epsilon)n/2$ against $X$. In other words $\payoffb(X,X) \geq (1-5\epsilon)n/2$. Since $Y$ is a best response of the follower against the leader's strategy, we have $\payoffb(X,Y) \geq \payoffb(X,X) \geq (1-5\epsilon)n/2$ and thus
    \begin{equation*}
    \begin{split}
    \mathbb{E}_{x \sim X} [\common(x,Y)] & = \payoffb(X,Y) \\
    & \geq \payoffb(X,X)\\
    & =  \mathbb{E}_{x \sim X, x' \sim X} [\common(x,x')]\\
    & \geq (1-5\epsilon)n/2.
    \end{split}
    \end{equation*}
    Hence
    \begin{equation}\label{fact3}
    \begin{split}
    \mathbb{E}_{x \sim X} [\dist(x,Y)] & = \mathbb{E}_{x \sim X} [|x| + |Y| - 2\common(x,Y)] \\
    & \leq \mathbb{E}_{x \sim X} [n - 2\common(x,Y)]\\
    & = n-2\mathbb{E}_{x \sim X} [\common(x,Y)]\\
    & \leq n-2(1-5\epsilon)n/2\\
    & \leq 5\epsilon n
    \end{split}
    \end{equation}
    Combining Inequalities \eqref{fact1} and \eqref{fact3} yields
    \begin{equation*}
    \dist(Y, Y^*) \leq \mathbb{E}_{x \sim X} [\dist(x,Y)] + \mathbb{E}_{x \sim X} [\dist(x,Y^*)] \leq 6\epsilon n.
    \end{equation*}
    Therefore, we have $\common(Y, Y^*) \geq |Y^*|- 6\epsilon n$ and since $|Y^*| \geq (1-\epsilon)n/2$ we have $\common(Y, Y^*) \geq (1-13\epsilon)n/2  >  (1-\epsilon')n/2$. Now, if the solution of $\I$ is not $n/2$, then it is at most $(1-\epsilon')n/2$. Therefore, $\common(Y, Y^*) > (1-\epsilon')n/2$ happens if and only if the solution of $I$ is exactly $n/2$. Thus, an approximation solution for $\cori$ within a factor $(1-\epsilon) > (1-\epsilon'/13)$ can be used to decide if the solution of $\I$ is $n/2$ or bounded by $(1-\epsilon')n/2$. This implies a hard gap for the \matchingproblem\enspace problem at gap location $1$.
\end{proof}

All that remains is to prove the statement of Lemma \ref{lm1} and that completes the proof Theorem \ref{apxhardness}.

\begin{proof}[of Lemma \ref{lm1}]
    \input{figs/reduction1.tex}
    We show this lemma by a reduction from the \threedM\enspace problem. In \threedM\enspace problem, we are given a hypergraph $G$ whose vertices are divided into three parts $A$, $B$, and $C$. Every edge of $G$ is a triple $(a,b,c)$ of the vertices such that $a \in A$, $b \in B$, and $c \in C$ hold. A matching in this graph is a subset of the edges that do not share any vertices. The goal of the problem is to find a matching with the maximum number of edges. \petrankhardness~\cite{petrank1994hardness} showed that the \threedM\enspace problem has a hard gap at gap location $1$.
    
    We show via a reduction that \matchingproblem\enspace is harder than the \threedM\enspace problem. This implies a similar hardness result for the \matchingproblem\enspace problem. To this end, suppose we are given an instance $\I$ of the 3-dimensional matching problem. Let the graph of this instance be $G$ and its vertices lie in three parts $A$, $B$, and $C$ such that every edge of the graph contains a vertex of each part. We construct a bipartite graph $G'$ and a function $\pi$ based on $G$ as follows:
    \begin{itemize}
        \item $G'$ contains two independent parts $X$ and $Y$, each of which contains an endpoint of every edge of the graph.
        \item $X = A' \cup A''$ where  $A'$ and $A''$ are two copies of $A$.
        \item $Y = B' \cup C'$ where $B'$ is a copy of $B$ and $C'$ is a copy of $C$.
        \item For every vertex $a \in A$, we put two vertices $a'$ and $a''$ in $X$ (in $A'$ and $A''$ respectively).
        \item For every vertex $b \in B$ we put a vertex $b'$ in $Y$ (in part $B'$).
        \item For every vertex $c \in C$ we put a vertex $c'$ in $Y$ (in part $C'$).
        \item For every edge $(a,b,c)$ of $G$, we put two edges $(a',b')$ and $(a'',c')$ in $G'$. Moreover, we set $\pi((a',b')) = (a'',c')$ and $\pi((a'',c')) = (a',b')$. Note that this way, there may be multiple edges between two vertices of $G$ with different $\pi$ values.
    \end{itemize}
    Now, we argue that for every 3-dimensional matching $M$ of $G$, there exists a matching $M'$ of $G'$ such that $|M' \cap \pi(M')| = 2|M|$ and viceversa. To this end, suppose $M$ is a 3-dimensional matching of $G$. Now, we set $M' = \{(a,b,c) \in E(G) | (a',b')\} \cup \{(a,b,c) \in E(G) | (a'',c')\}$. Since $M$ is a matching, no two edges of $M'$ share a vertex and thus $M'$ is also a matching. Moreover, for every edge in $M'$, its $\pi$ transformation is also included in $M'$ and therefore $M' = \pi(M')$. Hence $|M' \cap \pi(M')| = |M'| = 2|M|$. A similar argument shows that for any matching $M'$ of $G'$ such that $|M' \cap \pi(M')| = 2k$, there exists a matching of size $k$ in $G$. Therefore, the problem of finding a maximum 3-dimensional matching of $G$ reduces to finding a matching of $G'$ that shares the maximum number of edges with its $\pi$-transformation. Since \threedM\enspace problem has a hard gap at gap location $1$, so does the \matchingproblem\enspace problem. Figure \ref{reduction1} describes the reduction mentioned above.
\end{proof}
\subsection{A $1/12$ Approximation Solution}
In Section \ref{section:apx}, we showed that approximating an SE of the \mgame\  game within an arbitrarily small error is NP-hard. We complement this result by presenting a polynomial time algorithm to compute a $1/12$-approximation solution. In other words, our algorithm provides a strategy $X$ for the leader that achieves at least a $1/12$ fraction of the payoff of an SE against the best response of his opponent.

We first devise a greedy algorithm to find two matchings $x$ and $x'$ such that $x$ shares as many edges as possible with the $\pi$-transformation of $x'$. To this end, we begin with two empty matchings $x$ and $x'$ and every time choose two edges $e$ and $e'$ of the graph such that $\pi(e') = e$, $e$ is not adjacent\footnote{two edges are adjacent if they share a common vertex.} to any edge of $x$, and $e'$ is not adjacent to any edge of $x'$. Next, we update the matchings by adding $e$ to $x$ and $e'$ to $x'$.

\begin{algorithm}
    \label{alg:matchings}
    \KwData{A graph $G$ and a one-to-one mapping $\pi$ over the edges of $G$.}
    \KwResult{Two matchings $x$ and $x'$.}
    $x \leftarrow \emptyset$\;    
    $x' \leftarrow \emptyset$\;
    \While{\text{there exist edges $e$ and $e'$ s.t} \begin{itemize}
                \item $e = \pi(e')$
                \item \text{$e$ doesn't share any vertices with $x$}
                \item \text{$e'$ doesn't share any vertices with $x'$}
            \end{itemize}}{
            \text{Add $e$ to $x$}\;
            \text{Add $e'$ to $x'$}\;
    }
    \textbf{Return}$(x,x')$\;
    \caption{Maximizing the number of edges that $x$ shares with $\pi(x')$}
\end{algorithm}

We show that Algorithm \ref{alg:matchings} obtains a $1/4$ approximation solution. Let $x$ and $x'$ be the matchings provided by Algorithm \ref{alg:matchings} and suppose for the sake of contradiction that there exist two matchnigs $y$ and $y'$ such that $\common(y,\pi(y')) > 4\common(x,\pi(x'))$. Due to Algorithm \ref{alg:matchings}, we have $|x| = |x'| = \common(x,\pi(x'))$. Moreover, there are at least $4\common(x,\pi(x'))$ edges in $y'$ whose $\pi$-transformations appear in $y$. Notice that for every edge $e'$ in $x'$, there are at most four of such edges in $y'$ such that either share an end-point with $e'$ or their $\pi$-transfrmations share an endpoint with $\pi(e')$. Thus, there exists an edge $e'$ in $y$ such that neither $e'$ shares a vertex with the vertices of $x'$ nor $\pi(e')$ shares an endpoint with the vertices of $x$. This is a contradiction since our algorithm terminates when no such pair of edges exists. This observation implies that $|x \cap \pi(x')|$ is at least $1/4$ fraction of the payoff of the leader in any SE.

\begin{observation}\label{observation:matchings}
    Let $x$ and $x'$ be the matchings determined by Algorithm \ref{alg:matchings}. $|x \cap \pi(x')|$ is at least $1/4$ fraction of the optimal payoff the leader gets in an SE.
\end{observation}
\begin{proof}
    Recall that the payoff of the leader is the number of edges his matching has in common with the $\pi$-transformation of the follower's matching. This value is always upper bounded by $4|x \cap \pi(x')|$ for any pair of matchings and thus the proof is complete.
\end{proof}

Let $\epsilon > 0$ be an arbitrarily small positive number and $X$ be a strategy of the leader that plays matching $x$ with probability $1/3-\epsilon$ and matching $x'$ with probability $2/3+\epsilon$. Moreover, let $Y$ be a best response of the follower against $X$. Based on Observation \ref{observation:matchings}, we show that $\payoffa(X,Y)$ is at least $(1-3\epsilon)/12$ fractional of the optimal payoff the leader can get in any SE.

\begin{theorem}
    Let $X$ and $Y$ be the strategies of the leader and the follower defined above. $\payoffa(X,Y)$ is at least $(1-3\epsilon)/12$ fraction of the optimal payoff the leader achieves in any SE.
\end{theorem}
\begin{proof}
    We assume w.l.g that $Y$ is a pure strategy. We first show that $Y$ contains all edges of $x'$. To this end, suppose for the sake of contradiction that an edge $e'$ of $x'$ doesn't appear in $Y$. If we add this edge to $Y$ and remove the edges of $Y$ that share an endpoint with $e'$ then the payoff of the follower changes as follows: Because $X$ plays $x'$ with probability $2/3+\epsilon$ then  $e'$ appears in his strategy with probability $2/3+\epsilon$ and thus the payoff of the follower is increased by $2/3+\epsilon$. Moreover, none of the crossing edges of $e'$ with edges of $Y$ are in $x'$ and thus appear in the leader's strategy with probability at most $1/3-\epsilon$. This incurs a loss of at most $2(1/3-\epsilon) < 2/3+\epsilon$. Thus, this change improves the payoff of the follower which shows $Y$ is not a best response against $X$ which is a contradiction.
    
    Note that $X$ plays $x$ with probability $1/3-\epsilon$ and $Y$ contains every edge of $x'$. Thus, the payoff of the leader is at least $$(1/3-\epsilon)\payoffa(x,x') = (1/3-\epsilon) \common(x,\pi(x')) = (1-3\epsilon) \common(x,\pi(x'))/3.$$ This along with the fact that the payoff of the leader in any SE is at most $4\common(x,\pi(x'))$ (Observation \ref{observation:matchings}) proves that $\payoffa(x,y)$ is at least a $(1-3\epsilon)/12$ fraction of the optimal payoff the leader achieves in any SE.
\end{proof}

==> sources/apxhardness_ew.tex <==


\section{The \mgame\ Game}\label{section:apx}

\nhedit{In this section, we introduce a large but structured Stackelberg game, \mgame, and examine the computational complexity of computing its Stackelberg equilibrium. We show two sets of results for this game. In Section~\ref{section:apx}, we show the existing structure in \mgame is not sufficient for efficient computation of  Stackelberg equilibrium  -- we show that this problem is APX-hard. In Section~\ref{sec:mgame-approx}, we give an efficient $\frac 12$ approximation.

Here, let us highlight an important aspect of our hardness results in advance. As we will show, the strategy space of the players in \mgame Game, though large, is very structured. At a high level, the reward of each player is a linear function of the action of the other and each player can optimize a linear function over the strategy of the other player, for example, each player can compute a best-response  to a mixed strategy of the other. In a zero-sum game, existence of such a structure leads to efficient algorithms for computing the Nash or Stackelberg equilibria~\cite{ahmadinejad2016duels, DHL+17, KV05}. On the other hand, our APX-hardness result for the \mgame game shows that existence of this structure does not necessarily lead to efficient algorithms for computing Stackelberg equilibira in general-sum games. 

With this in mind, let us describe the \mgame games as follows. Consider a multigraph $G$, a one-to-one mapping $\pi: E(G) \rightarrow E(G)$ over the edges of $G$ and two players $A$ and $B$ taking the roles of the leader and follower, respectively.
For a set $S$ of the edges of $G$, we define $\pi(S) = \{e \in S| \pi(e)\}$ and assume $\pi(S) = T \Leftrightarrow \pi^{-1}(T) = S$. Note that we assume that $G$ is a multigraph and may contain parallel edges between a pair of vertices. In this case, the $\pi$ values for two parallel edge may differ. In thes rest of this section, every time we use the term graph we refer to a multigraph. Each player's pure strategy is a matching of $G$ and for two matching $M_A$ and $M_B$ for players $A$ and $B$ we define the payoffs of the players as follows:
\begin{equation*}
\payoffa(M_A,M_B) = |M_A \cap \pi(M_B)| \hspace{2cm} \payoffb(M_A,M_B) = |M_A \cap M_B|
\end{equation*} 

Note that $G$ and $\pi$ are known to both players in advance. We refer to player $A$ as leader and call player $B$ the follower.

}

\subsection{Hardness of approximation}
%\nhcomment{The first three paragraphs are redundant now that we have the full introduction. I think we should remove it. Add a subsection for hardness of approximation}

%In this section, we discuss the computational complexity of determining the Stackelberg equilibria of huge games. It has been shown that a Stackelberg equilibrium of a game can be found in polynomial time when the follower has polynomially many pure strategies~\cite{paruchuri2008playing}. Note that since the follower always plays a best response in an SE, we can assume w.l.g that the strategy of the follower in an SE is always pure. Therefore, one could iterate over all possible pure strategies of the follower and solve the problem subject to follower's best-response being a fixed pure strategy. To this end, for a fixed pure strategy $Y$ of the follower, we wish to find a strategy $X$ (possibly mixed) of the leader such that (i) $Y$ is a best-response against $X$ and (ii) $X$ maximizes the payoff of the leader against $Y$. Indeed both criteria can be formulated with linear constraints and thus this problem can be modeled with an LP~\cite{paruchuri2008playing}. Thus, an SE of a game can be determined by solving an LP for each pure strategy of the follower and taking the maximum payoff of the leader over all solutions. However, the running time of this solution depends linearly on the number of pure strategies of the follower and thus it does not run in polynomial time when the follower has exponentially many pure strategies.

%Although the problem is trivially intractable when any of the players has exponentially many pure strategies due to the massive input length, it still remains a question whether the problem admits a fast solution for \textit{structured games}. For instance, one could define a game in which players' strategies are the set of all matchings or spanning trees of a graph. As such, the input to the problem is only a graph which is polynomially representable, nonetheless, the players have exponentially many pure strategies. Several recent works aimed at studying the computational complexity of finding an NE of such games~\cite{immorlica2011dueling,ahmadinejad2016duels,behnezhad2016faster,garg2011bilinear,xu2016mysteries,wang2017security}. For instance, the classic approach for computing the equilibria of a two player zero-sum game fails when the players have exponentially many pure strategies. However, \ahmadinejadduels~\cite{ahmadinejad2016duels} prove that it only suffices to be able to optimize a linear function over the strategies of the players in polynomial time to compute the equilibria of a two player zero-sum game in polynomial time. This result holds for all two player zero-sum games regardless of the size of the strategies. Notice that NE and SE are equivalent concepts for zero-sum games~\cite{korzhyk2011stackelberg}, and as such, their result can be seen as a solution for Stackelberg equilibria for the special case of zero-sum games. A natural question that emerges here is whether a similar algorithm can be designed to compute or even approximate an SE of a structured but non-zero-sum game. In what follows, we show that the answer is negative unless P=NP.


The goal of this section is to show a hardness result for the Stackelberg equilibria of large structured games. In contrast to the zero-sum setting, we prove that a polynomial time algorithm for optimizing the strategies in a Stackelberg game does not necessarily lead to a polynomial time solution for Stackelberg equilibria. More precisely, we show that in some cases, the problem of (approximately) computing a Stackelberg equilibrium of a game is NP-hard even if optimization over the strategy space of the players is polynomially tractable.

To this end, we present a game such that any linear function over the strategies of this game can be optimized in polynomial time. Next, we proceed by showing that finding an SE of this game is NP-hard. Moreover, we show that the problem remains hard, even if we wish to approximate an SE of the game within a small error.


%We define the \textit{\mgame\  game} as follows: In a \mgame\  game, we have a graph $G$, an injective surjective (one-to-one) function $\pi: E(G) \rightarrow E(G)$ over the edges of $G$ and two players $A$ and $B$. For a set $S$ of the edges of $G$, we define $\pi(S) = \{e \in S| \pi(e)\}$ and assume $\pi(S) = T \Leftrightarrow \pi^{-1}(T) = S$. Note that we assume that $G$ is a multigraph and may contain parallel edges between a pair of vertices. In this case, the $\pi$ values for two parallel edge may differ. In thes rest of this section, every time we use the term graph we refer to a multigraph. Each player's pure strategy is a matching of $G$ and for two matching $M_A$ and $M_B$ for players $A$ and $B$ we define the payoffs of the players as follows:
%\begin{equation*}
%\payoffa(M_A,M_B) = |M_A \cap \pi(M_B)| \hspace{2cm} \payoffb(M_A,M_B) = |M_A \cap M_B|
%\end{equation*} 

%\begin{center}
%    \noindent\framebox{\begin{minipage}{6.50in}
%            \textsf{\mgame\ }\\[0.25cm]
%            \textsf{Input}: An unweighted undirected graph $G$ and an injective surjective function $\pi$ over the edges of $G$. \\[0.25cm]
%            \textsf{Players strategies:} Each players pure strategies is the set of all matchings of $G$.\\[0.25cm]
%            \textsf{Player $A$'s payoff:} The number of edges his matching has in common with the $\pi$-transformation of player $B$'s matching.\\[0.25cm]
%            \textsf{Player $B$'s payoff:} The number of edges his matching has in common with player $A$'s matching.\\[0.25cm]
%    \end{minipage}}
%\end{center}

Note that $G$ and $\pi$ are known to both players in advance. We refer to player $A$ as leader and call player $B$ the follower. Each strategy of the players in this game can be represented with a 0-1 vector of size $|E(G)|$ whose every element specifies whether a particular edge appears in the matching. We first show that the strategies of both players can be optimized with respect to any linear function over the edges of the graph.


%\red{[NH: Add the zero-sum version of the results in a theorem environment.]}

\begin{observation}\label{salam1}
    There exists a polynomial time algorithm such that for every vector $w$ of size $|E(G)|$ finds a strategy of the players whose corresponding representation vector $v$ maximizes $v.w$.
\end{observation}
\begin{proof}
    This problem reduces to finding a maximum weighted matching of a graph. We associate a weight $w_e$ to every edge $e$ of the graph which is equal to the value of the corresponding element of $e$ in vector $w$. Now, the weight of any matching in this graph is equal to the dot product of $w$ and the representation vector of the matching and thus the problem reduces to finding the maximum weighted matching of the graph which can be done in polynomial time ~\cite{cormen2009introduction}.
\end{proof}

Recall that Observation \ref{salam1} is enough for the framework of \ahmadinejadduels~\cite{ahmadinejad2016duels} to show that an NE (or equivalently an SE) of the game can be computed in polynomial time for a zero-sum variant of the game. However, as we show, this property alone does not guarantee a polynomial time solution for the case of Stackelberg equilibria of non-zero-sum games.
In what follows we show that it is impossible to approximate a Stackelberg equilibrium of the \mgame\  game in polynomial time within an arbitrarily small constant factor unless P=NP.

Before we proceed to the proof, we define an auxiliary problem and show a hardness result for this problem. Later we take advantage of this hardness result to show an APX-hardness result for finding a Stackelberg equilibrium of the \mgame\  game. To this end, we define \textit{the \matchingproblem\enspace problem} as follows:

\begin{center}
    \noindent\framebox{\begin{minipage}{6.50in}
            \textsf{\matchingproblem\enspace}\\[0.25cm]
            \textsf{Input}: An unweighted undirected graph $G$ and an injective surjective function $\pi: E(G) \rightarrow E(G)$ over the edges of $G$. \\[0.25cm]
            \textsf{Output:} A matching $M$ of $G$ such that $|M \cap \pi(M)|$ is maximized.\\[0.25cm]
    \end{minipage}}
\end{center}

We show that \matchingproblem\enspace has a \textit{hard gap} at \textit{gap location $1$}. In other words, it is NP-hard to decide whether for a given graph $G$ with $n$ vertices and a function $\pi$, the solution of the \matchingproblem\enspace problem is exactly equal to $n/2$ or at most $(1-\epsilon)n/2$ for some $\epsilon > 0$.

\begin{lemma}\label{lm1}
    There exists an $\epsilon > 0$ such that it is NP-hard to decide whether the solution of the \matchingproblem\enspace problem is exactly equal to $n/2$ or less than $(1-\epsilon)n/2$ where $n$ is the number of the vertices of the input graph.
\end{lemma}
Another way to phrase Lemma \ref{lm1} is that the \matchingproblem\enspace problem has a hard gap at gap location 1. For brevity, we skip the proof of Lemma \ref{lm1} here and defer it to the end of this section. Based on Lemma \ref{lm1}, we are now ready to prove the main result of this section.

\begin{theorem}\label{apxhardness} \label{thm:apxhardness}
    Computing a Stackelberg equilibrium of the \mgame\  game is APX-hard.
\end{theorem}
\begin{proof}
    More generally we show that approximating a Stackelberg equilibrium of the \mgame\  game has a hard gap at gap location $1$. This immediately implies a hardness of approximation. We show this by a reduction from the \matchingproblem\enspace problem. Suppose we are given an instance $\I = \langle G, \pi\rangle$ of the \matchingproblem\enspace problem and wish to decide for some $\epsilon' > 0$, whether the solution of this problem is exactly $n/2$ or it is bounded by $(1-\epsilon')n/2$ where $n$ is the size of $G$.
    Based on $\I$, we construct an instance $\cori$ of the \mgame\  game with the same graph $G$ and transformation function $\pi$ and seek to find a Stackelberg equilibrium of the leader (player $A$) in this game. Note that by definition, the solution of $\I$ is equal to $n/2$ if and only if $G$ contains a perfect matching which is identical to its $\pi$-transformation. Otherwise, the solution of $\I$ is at most $(1-\epsilon')n/2$ and thus any matching of $G$ shares no more than $(1-\epsilon')n/2$ edges with its $\pi$-transformation.
    
    Since for small enough $\epsilon'$ it is NP-hard to distinguish the two cases (Lemma \ref{lm1}), we show that it is NP-hard to approximate a Stackelberg equilibrium of the leader in $\cori$. If the solution of $\I$ is $n/2$, then there exists a perfect matching in $G$ which is identical to its $\pi$-transformation. Thus, if both players play this matching in $\cori$, they both get a payoff of $n/2$ and since $n/2$ is the maximum possible payoff for any player in this game, this makes the game a Stackelberg equilibrium for the leader. Therefore, in this case, the leader achieves a payoff of $n/2$ in a Stackelberg equilibrium of the \mgame\  game. 
    
    Now, suppose for $\epsilon < \epsilon'/13$ we have a $1-\epsilon$ approximation solution for $\cori$. If the solution of $\I$ is $n/2$, then the payoff of the leader in such an approximation solution is at least $n(1-\epsilon)/2$. Let the strategies of the leader and follower be $X$ and $Y$ in this solution. Therefore, $\payoffa(X,Y) \geq n(1-\epsilon)/2$. Notice that $X$ may be a mixed strategy, but we can assume w.l.g that $Y$ is a pure strategy since there always exists a best response for the follower which is pure. Also, let $Y^*$ be the $\pi$-transformation of strategy $Y$. Let for two matchings $x$ and $y$, $\common(x,y)$ denote the number of edges that $x$ and $y$ have in common and define $\dist(x,y) = |x| + |y|-2\common(x,y)$. Recall that the payoff of player $A$ in this game can be formulated as $\mathbb{E}_{x \sim X} [\common(x,Y^*)]$. Since this value is at least $n(1-\epsilon)/2$ we have:
    \begin{equation*}
    \mathbb{E}_{x \sim X} [\common(x,Y^*)] = \payoffa(X,Y) \geq n(1-\epsilon)/2
    \end{equation*}
    and thus
    \begin{equation}\label{fact1}
    \begin{split}
    \mathbb{E}_{x \sim X} [\dist(x,Y^*)] & =  \mathbb{E}_{x \sim X} [|x| + |Y^*| - 2\common(x,Y^*)]\\
    & \leq  \mathbb{E}_{x \sim X} [n - 2\common(x,Y^*)]\\
    & = n - 2\mathbb{E}_{x \sim X} [\common(x,Y^*)]\\
    & \leq n - 2 n(1-\epsilon)/2\\
    & = n - n(1-\epsilon)\\
    & \leq n \epsilon.
    \end{split}
    \end{equation}
    Inequality \eqref{fact1} shows that $Y^*$ is very similar (in expectation) to a random matching drawn from strategy $X$. This intuitively implies that pure strategies of $X$ should have lots of edges in common. It follows from the definition that for three matchings $x$, $y$, and $z$ we have $\dist(x,z) \leq \dist(x,y) + \dist(y,z)$. Therefore, we have 
    \begin{equation}\label{fact2}
    \begin{split}
    \mathbb{E}_{x \sim X, x' \sim X} [\dist(x,x')] & \leq \mathbb{E}_{x \sim X, x' \sim X} [\dist(x,Y^*) + \dist(Y^*,x')]\\
    & = \mathbb{E}_{x \sim X, x' \sim X} [\dist(x,Y^*) + \dist(x', Y^*)]\\
    & = \mathbb{E}_{x \sim X} [\dist(x,Y^*)] + \mathbb{E}_{x' \sim X} [\dist(x',Y^*)]\\
    & = 2 \mathbb{E}_{x \sim X} [\dist(x,Y^*)]\\
    & \leq 2\epsilon n
    \end{split}
    \end{equation}
    Recall that the payoff of the follower is determined by the number of edges his matching shares with that of the leader. Recall that since $\payoffa(X,Y) \geq n(1-\epsilon)/2$, this implies that $\mathbb{E}_{x \sim X}[|x|] \geq n(1-\epsilon)/2$. What Inequality \eqref{fact2} implies is that if the follower plays $X$ instead of $Y$, he gets a payoff of at least $\mathbb{E}_{x \sim X}|x| - 2\epsilon n \geq (1-5\epsilon)n/2$ against $X$. In other words $\payoffb(X,X) \geq (1-5\epsilon)n/2$. Since $Y$ is a best response of the follower against the leader's strategy, we have $\payoffb(X,Y) \geq \payoffb(X,X) \geq (1-5\epsilon)n/2$ and thus
    \begin{equation*}
    \begin{split}
    \mathbb{E}_{x \sim X} [\common(x,Y)] & = \payoffb(X,Y) \\
    & \geq \payoffb(X,X)\\
    & =  \mathbb{E}_{x \sim X, x' \sim X} [\common(x,x')]\\
    & \geq (1-5\epsilon)n/2.
    \end{split}
    \end{equation*}
    Hence
    \begin{equation}\label{fact3}
    \begin{split}
    \mathbb{E}_{x \sim X} [\dist(x,Y)] & = \mathbb{E}_{x \sim X} [|x| + |Y| - 2\common(x,Y)] \\
    & \leq \mathbb{E}_{x \sim X} [n - 2\common(x,Y)]\\
    & = n-2\mathbb{E}_{x \sim X} [\common(x,Y)]\\
    & \leq n-2(1-5\epsilon)n/2\\
    & \leq 5\epsilon n
    \end{split}
    \end{equation}
    Combining Inequalities \eqref{fact1} and \eqref{fact3} yields
    \begin{equation*}
    \dist(Y, Y^*) \leq \mathbb{E}_{x \sim X} [\dist(x,Y)] + \mathbb{E}_{x \sim X} [\dist(x,Y^*)] \leq 6\epsilon n.
    \end{equation*}
    Therefore, we have $\common(Y, Y^*) \geq |Y^*|- 6\epsilon n$ and since $|Y^*| \geq (1-\epsilon)n/2$ we have $\common(Y, Y^*) \geq (1-13\epsilon)n/2  >  (1-\epsilon')n/2$. Now, if the solution of $\I$ is not $n/2$, then it is at most $(1-\epsilon')n/2$. Therefore, $\common(Y, Y^*) > (1-\epsilon')n/2$ happens if and only if the solution of $I$ is exactly $n/2$. Thus, an approximation solution for $\cori$ within a factor $(1-\epsilon) > (1-\epsilon'/13)$ can be used to decide if the solution of $\I$ is $n/2$ or bounded by $(1-\epsilon')n/2$. This implies a hard gap for the \matchingproblem\enspace problem at gap location $1$.
\end{proof}

All that remains is to prove the statement of Lemma \ref{lm1} and that completes the proof Theorem \ref{apxhardness}.

\begin{proof}[of Lemma \ref{lm1}]
    \input{figs/reduction1.tex}
    We show this lemma by a reduction from the \threedM\enspace problem. In \threedM\enspace problem, we are given a hypergraph $G$ whose vertices are divided into three parts $A$, $B$, and $C$. Every edge of $G$ is a triple $(a,b,c)$ of the vertices such that $a \in A$, $b \in B$, and $c \in C$ hold. A matching in this graph is a subset of the edges that do not share any vertices. The goal of the problem is to find a matching with the maximum number of edges. \petrankhardness~\cite{petrank1994hardness} showed that the \threedM\enspace problem has a hard gap at gap location $1$.
    
    We show via a reduction that \matchingproblem\enspace is harder than the \threedM\enspace problem. This implies a similar hardness result for the \matchingproblem\enspace problem. To this end, suppose we are given an instance $\I$ of the 3-dimensional matching problem. Let the graph of this instance be $G$ and its vertices lie in three parts $A$, $B$, and $C$ such that every edge of the graph contains a vertex of each part. We construct a bipartite graph $G'$ and a function $\pi$ based on $G$ as follows:
    \begin{itemize}
        \item $G'$ contains two independent parts $X$ and $Y$, each of which contains an endpoint of every edge of the graph.
        \item $X = A' \cup A''$ where  $A'$ and $A''$ are two copies of $A$.
        \item $Y = B' \cup C'$ where $B'$ is a copy of $B$ and $C'$ is a copy of $C$.
        \item For every vertex $a \in A$, we put two vertices $a'$ and $a''$ in $X$ (in $A'$ and $A''$ respectively).
        \item For every vertex $b \in B$ we put a vertex $b'$ in $Y$ (in part $B'$).
        \item For every vertex $c \in C$ we put a vertex $c'$ in $Y$ (in part $C'$).
        \item For every edge $(a,b,c)$ of $G$, we put two edges $(a',b')$ and $(a'',c')$ in $G'$. Moreover, we set $\pi((a',b')) = (a'',c')$ and $\pi((a'',c')) = (a',b')$. Note that this way, there may be multiple edges between two vertices of $G$ with different $\pi$ values.
    \end{itemize}
    Now, we argue that for every 3-dimensional matching $M$ of $G$, there exists a matching $M'$ of $G'$ such that $|M' \cap \pi(M')| = 2|M|$ and viceversa. To this end, suppose $M$ is a 3-dimensional matching of $G$. Now, we set $M' = \{(a,b,c) \in E(G) | (a',b')\} \cup \{(a,b,c) \in E(G) | (a'',c')\}$. Since $M$ is a matching, no two edges of $M'$ share a vertex and thus $M'$ is also a matching. Moreover, for every edge in $M'$, its $\pi$ transformation is also included in $M'$ and therefore $M' = \pi(M')$. Hence $|M' \cap \pi(M')| = |M'| = 2|M|$. A similar argument shows that for any matching $M'$ of $G'$ such that $|M' \cap \pi(M')| = 2k$, there exists a matching of size $k$ in $G$. Therefore, the problem of finding a maximum 3-dimensional matching of $G$ reduces to finding a matching of $G'$ that shares the maximum number of edges with its $\pi$-transformation. Since \threedM\enspace problem has a hard gap at gap location $1$, so does the \matchingproblem\enspace problem. Figure \ref{reduction1} describes the reduction mentioned above.
\end{proof}
\subsection{A $1/12$ Approximation Solution}
In Section \ref{section:apx}, we showed that approximating an SE of the \mgame\  game within an arbitrarily small error is NP-hard. We complement this result by presenting a polynomial time algorithm to compute a $1/12$-approximation solution. In other words, our algorithm provides a strategy $X$ for the leader that achieves at least a $1/12$ fraction of the payoff of an SE against the best response of his opponent.

We first devise a greedy algorithm to find two matchings $x$ and $x'$ such that $x$ shares as many edges as possible with the $\pi$-transformation of $x'$. To this end, we begin with two empty matchings $x$ and $x'$ and every time choose two edges $e$ and $e'$ of the graph such that $\pi(e') = e$, $e$ is not adjacent\footnote{two edges are adjacent if they share a common vertex.} to any edge of $x$, and $e'$ is not adjacent to any edge of $x'$. Next, we update the matchings by adding $e$ to $x$ and $e'$ to $x'$.

\begin{algorithm}
    \label{alg:matchings}
    \KwData{A graph $G$ and a one-to-one mapping $\pi$ over the edges of $G$.}
    \KwResult{Two matchings $x$ and $x'$.}
    $x \leftarrow \emptyset$\;    
    $x' \leftarrow \emptyset$\;
    \While{\text{there exist edges $e$ and $e'$ s.t} \begin{itemize}
                \item $e = \pi(e')$
                \item \text{$e$ doesn't share any vertices with $x$}
                \item \text{$e'$ doesn't share any vertices with $x'$}
            \end{itemize}}{
            \text{Add $e$ to $x$}\;
            \text{Add $e'$ to $x'$}\;
    }
    \textbf{Return}$(x,x')$\;
    \caption{Maximizing the number of edges that $x$ shares with $\pi(x')$}
\end{algorithm}

We show that Algorithm \ref{alg:matchings} obtains a $1/4$ approximation solution. Let $x$ and $x'$ be the matchings provided by Algorithm \ref{alg:matchings} and suppose for the sake of contradiction that there exist two matchnigs $y$ and $y'$ such that $\common(y,\pi(y')) > 4\common(x,\pi(x'))$. Due to Algorithm \ref{alg:matchings}, we have $|x| = |x'| = \common(x,\pi(x'))$. Moreover, there are at least $4\common(x,\pi(x'))$ edges in $y'$ whose $\pi$-transformations appear in $y$. Notice that for every edge $e'$ in $x'$, there are at most four of such edges in $y'$ such that either share an end-point with $e'$ or their $\pi$-transfrmations share an endpoint with $\pi(e')$. Thus, there exists an edge $e'$ in $y$ such that neither $e'$ shares a vertex with the vertices of $x'$ nor $\pi(e')$ shares an endpoint with the vertices of $x$. This is a contradiction since our algorithm terminates when no such pair of edges exists. This observation implies that $|x \cap \pi(x')|$ is at least $1/4$ fraction of the payoff of the leader in any SE.

\begin{observation}\label{observation:matchings}
    Let $x$ and $x'$ be the matchings determined by Algorithm \ref{alg:matchings}. $|x \cap \pi(x')|$ is at least $1/4$ fraction of the optimal payoff the leader gets in an SE.
\end{observation}
\begin{proof}
    Recall that the payoff of the leader is the number of edges his matching has in common with the $\pi$-transformation of the follower's matching. This value is always upper bounded by $4|x \cap \pi(x')|$ for any pair of matchings and thus the proof is complete.
\end{proof}

Let $\epsilon > 0$ be an arbitrarily small positive number and $X$ be a strategy of the leader that plays matching $x$ with probability $1/3-\epsilon$ and matching $x'$ with probability $2/3+\epsilon$. Moreover, let $Y$ be a best response of the follower against $X$. Based on Observation \ref{observation:matchings}, we show that $\payoffa(X,Y)$ is at least $(1-3\epsilon)/12$ fractional of the optimal payoff the leader can get in any SE.

\begin{theorem}
    Let $X$ and $Y$ be the strategies of the leader and the follower defined above. $\payoffa(X,Y)$ is at least $(1-3\epsilon)/12$ fraction of the optimal payoff the leader achieves in any SE.
\end{theorem}
\begin{proof}
    We assume w.l.g that $Y$ is a pure strategy. We first show that $Y$ contains all edges of $x'$. To this end, suppose for the sake of contradiction that an edge $e'$ of $x'$ doesn't appear in $Y$. If we add this edge to $Y$ and remove the edges of $Y$ that share an endpoint with $e'$ then the payoff of the follower changes as follows: Because $X$ plays $x'$ with probability $2/3+\epsilon$ then  $e'$ appears in his strategy with probability $2/3+\epsilon$ and thus the payoff of the follower is increased by $2/3+\epsilon$. Moreover, none of the crossing edges of $e'$ with edges of $Y$ are in $x'$ and thus appear in the leader's strategy with probability at most $1/3-\epsilon$. This incurs a loss of at most $2(1/3-\epsilon) < 2/3+\epsilon$. Thus, this change improves the payoff of the follower which shows $Y$ is not a best response against $X$ which is a contradiction.
    
    Note that $X$ plays $x$ with probability $1/3-\epsilon$ and $Y$ contains every edge of $x'$. Thus, the payoff of the leader is at least $$(1/3-\epsilon)\payoffa(x,x') = (1/3-\epsilon) \common(x,\pi(x')) = (1-3\epsilon) \common(x,\pi(x'))/3.$$ This along with the fact that the payoff of the leader in any SE is at most $4\common(x,\pi(x'))$ (Observation \ref{observation:matchings}) proves that $\payoffa(x,y)$ is at least a $(1-3\epsilon)/12$ fraction of the optimal payoff the leader achieves in any SE.
\end{proof}
